Towards Large-Scale Autonomous Wireless Sensor Networks

Wireless Sensor Networks (WSNs) have the goal of gathering data from the environment. The advent of the Internet of Things (IoT) drastically changed WSN's vision that, as never before, needs to expand and include hundreds or thousands of sensors. But to follow the current IoT trends new techniques need to be implemented since orders of thousands of sensor nodes are not manageable by today's WSNs systems that often rely on manual configuration and hence are not practical. As an example, the replacement of batteries of thousand of nodes could be extremely arduous or even impossible for structural health monitoring of civil infrastructures (i.e. bridges, towers). Hence, the solution to the growing burden of the system manager is automation, allowing the system to check its own status, to re-configure itself and fix the major problems in the network whenever it is possible. In this paper, we present and discuss the main features needed to achieve an autonomous large scale WSN. Furthermore, we compare these features with the state of the art of real-world large scale WSN deployments showing that further solutions are needed to drastically reduce human intervention while guaranteeing the main functionalities of the system.

==> Capitoli/Conclusion.tex <==
%************************************************
\section{Conclusion and Future Work}
\label{sec:conclusion}
%************************************************
In this paper we present the feeatures that are still missing work towards a self sustainable wsn that reduce the human intervention to zero.
